Democratising Agricultural Commodity Price Forecasting: The AGRICAF Approach

Ensuring food security is a critical global challenge, particularly for low-income countries where food prices impact the access to nutritious food. The volatility of global agricultural commodity (AC) prices exacerbates food insecurity, with international trade restrictions and market disruptions further complicating the situation. Despite online platforms for monitoring food prices, there is a significant gap in providing detailed explanations and forecasts accessible to non-specialists. To address this, we propose the Agricultural Commodity Analysis and Forecasts (AGRICAF) methodology, integrating explainable machine learning (XML) and econometric techniques to analyse and forecast global agricultural commodity prices up to one year ahead, dynamically adapting to different forecast horizons. This innovative integration allows us to model complex interactions and dynamics while providing clear, interpretable results. This paper demonstrates how AGRICAF can be used, applying it to three major agricultural commodities - maize, soybean, and wheat - and explaining how different factors impact prices across various months and forecast horizons. By facilitating access to accurate and interpretable medium-term forecasts of AC prices, AGRICAF can contribute to developing a fair and sustainable food system.

==> 11_policy_implications.tex <==
%\section{Policy Implications}
High-income countries often have systems to enhance market transparency and manage price stability through information access, whereas low-income countries frequently experience sharp local price increases during crises, worsening food insecurity due to their limited resources and market information \citep{headey2008anatomy}. %To help closing the gap for low income countries, AGRICAF methodology will be made open source.
%AGRICAF is a novel forecasting methodology that combines XML and econometric techniques to generate medium-term agricultural commodity price forecasts. 
By offering clear, interpretable forecasts, AGRICAF aims to close gap to support a range of users—policymakers, smallholder farmers, cooperatives, and local community leaders—in better understanding anticipated price movements. 

For policymakers, AGRICAF could serve as a resource to help design more responsive food security policies, supporting efforts to stabilise food prices or manage strategic reserves during volatile periods. Smallholder farmers and cooperatives can use AGRICAF's forecasts to plan planting, storage, and sales, enabling them to plan market risks more effectively. Additionally, by making reliable, data-driven forecasts openly available, AGRICAF supports a more equitable global food system where low-income communities have improved access to essential market information, protecting them from severe price fluctuations that compromise their nutritional and economic well-being \citep{headey2023higher, barrett2011whyfood}.

On a high level, AGRICAF’s accessible price forecasts may contribute to Sustainable Development Goals (SDGs), particularly those focused on food security (SDG 2) and social equity (SDG 10) \citep{un2015transforming}. By enabling accessible agricultural commodity price forecasts, AGRICAF can assist policymakers to stabilise price and food supply more effectively, especially in low-income regions prone to food insecurity. 
With such knowledge, governments can proactively to manage reserves; implement price-stabilisation mechanisms to protect consumers from sudden price shocks; or inform farmers about expected price trends, risks and opportunities for the coming year.

AGRICAF also has implications for smallholder farmers and local community networks, such as NGOs and farmer cooperatives. AGRICAF can empower these agents to make informed decisions on planting, storage, and sales, therefore building greater resilience to price shifts. Smallholders can better navigate the market, optimise and negotiate better income, and reduce risks associated with unfamiliarity with the market conditions \citep{ferris2014linking, nxumalo2019determinants}. Intermediaries such as government agencies and NGOs can use AGRICAF to extend forecast information to rural areas, thus expanding the reach of these forecasts to farmers who may not have direct access \citep{adjemian2012emergence,abbott2016valuing}.

In addition to accessibility, AGRICAF emphasises transparency through its XML models, making it more trustworthy for non specialist users \citep{molnar2022} for crisis management and yearly policy planning. With its capacity for monthly updates, policymakers can respond regularly to evolving conditions, such as geopolitical crises or extreme weather events. This adaptability allows AGRICAF to support flexible policy adjustments, offering a tool for managing food supply and price stability in unstable times.

While the long-term policy impacts of AGRICAF remain to be fully evaluated, its accessible approach offers a potentially valuable tool for enhancing market transparency and resilience. By equipping policymakers and smallholder farmers with accessible, data-informed insights, AGRICAF may represent a step forward in addressing the structural challenges that contribute to market instability and food insecurity in low-income settings.

==> tabs/main_events.tex <==
\section*{Impact of Events on Global Prices of Maize, Soybean, and Wheat}

\subsection*{Maize}
\begin{enumerate}
    \item \textbf{2015-2016: El Niño Impact} \\
    \emph{Impact:} Severe weather conditions associated with El Niño led to droughts and floods, reducing global maize supply and increasing prices. \\
    \emph{Reference:} \cite{el_nino_impact}

    \item \textbf{2018: U.S.-China Trade Tensions} \\
    \emph{Impact:} Trade tensions between the U.S. and China disrupted agricultural trade patterns, causing fluctuations in maize prices. \\
    \emph{Reference:} \cite{us_china_trade_tensions}
\end{enumerate}


\subsection*{Rice}
\begin{enumerate}
    \item \textbf{2016-2017: Climate Events in Southeast Asia} \\
    \emph{Impact:} Climate events, such as typhoons and floods in Southeast Asia, can disrupt rice production. Reduced yields in major rice-producing countries in the region, like Vietnam and Thailand, contribute to a decrease in global rice supply, impacting prices. \\
    \emph{Reference:} \cite{}

    \item \textbf{2018:  Indian Export Policies} \\
    \emph{Impact:} Changes in export policies by major rice-producing countries, particularly India, can influence global rice prices. Export restrictions or policy shifts in India affect the availability of Indian rice in the international market, influencing price dynamics. \\
    \emph{Reference:} \cite{}
\end{enumerate}


\subsection*{Soybean}
\begin{enumerate}
    \item \textbf{2015-2016: El Niño Impact} \\
    \emph{Impact:} El Niño-induced weather events reduced soybean production globally, leading to higher soybean prices. \\
    \emph{Reference:} \cite{el_nino_impact}

    \item \textbf{2019-2020: U.S.-China Phase One Trade Deal} \\
    \emph{Impact:} The Phase One Trade Deal increased Chinese purchases of U.S. soybeans, positively impacting global soybean prices. \\
    \emph{Reference:} \cite{us_china_phase_one}
\end{enumerate}

\subsection*{Wheat}
\begin{enumerate}
    \item \textbf{2016: Russian Wheat Export Ban} \\
    \emph{Impact:} Russia's export ban on wheat reduced global supply, leading to higher wheat prices. \\
    \emph{Reference:} \cite{russian_wheat_ban}

    \item \textbf{2017: Australia Faces Production Challenges} \\
    \emph{Impact:} Production challenges in Australia, a major wheat exporter, decreased global wheat supply and increased prices. \\
    \emph{Reference:} \cite{australia_production_challenges}
\end{enumerate}

\subsection*{Additional Events}
\begin{enumerate}
    \item \textbf{2014-2015: Russia-Ukraine Conflict} \\
    \emph{Impact:} The conflict disrupted wheat production in the region, contributing to fluctuations in global wheat prices. \\
    \emph{Reference:} \cite{russia_ukraine_conflict}

    \item \textbf{2019-2020: COVID-19 Pandemic} \\
    \emph{Impact:} The pandemic disrupted supply chains and market demand, influencing global commodity prices, including maize, soybean, and wheat. \\
    \emph{Reference:} \cite{covid19_pandemic}
\end{enumerate}

